Autonomy for Ferries and Harbour Buses: a Collision Avoidance Perspective

This paper provides a collision avoidance perspective to maritime autonomy, in the shift towards Maritime Autonomous Surface Ships (MASS). In particular, the paper presents the developments related to the Greenhopper, Denmark's first autonomous harbour bus. The collision and grounding avoidance scheme, called the Short Horizon Planner (SHP), is described and discussed in detail. Furthermore, the required autonomy stack for facilitating safe and rule-compliant collision avoidance is presented. The inherent difficulties related to adhering to the COLREGs are outlined, highlighting some of the operational constraints and challenges within the space of autonomous ferries and harbour buses. Finally, collision and grounding avoidance is demonstrated using a simulation of the whole Greenhopper autonomy stack.

==> colregs_tikz.tex <==



% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_yfxndt14e}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_yfxndt14e}
{\pgfqpoint{0pt}{0pt}}
{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_ad2uj7z6h}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_ad2uj7z6h}
{\pgfqpoint{0pt}{0pt}}
{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_3evgjc7wg}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_3evgjc7wg}
{\pgfqpoint{0pt}{0pt}}
{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_y0hgzn6lm}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_y0hgzn6lm}
{\pgfqpoint{0pt}{0pt}}
{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,530); %set diagram left start at 0, and has height of 530

%Curve Lines [id:da9090519384981124] 
\draw    (175.33,227.79) .. controls (218.88,227.88) and (224.77,263.93) .. (257.06,264.86) ;
\draw [shift={(259.6,264.86)}, rotate = 178.45] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da3825534900198091] 
\draw    (247.8,228.46) .. controls (204.26,228.37) and (198.36,192.32) .. (166.07,191.38) ;
\draw [shift={(163.54,191.38)}, rotate = 358.45] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da20132192727982057] 
\draw    (330.85,189.95) -- (375.89,189.77) ;
\draw [shift={(327.85,189.96)}, rotate = 359.78] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7159013623089907] 
\draw    (346.02,260.18) .. controls (344.02,204.56) and (439.07,263.79) .. (439.11,192.17) ;
\draw [shift={(439.08,189.96)}, rotate = 88.54] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Pentagon Arrow [id:dp9558572100938112] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (132.36,219.78) -- (166.07,219.78) -- (175.33,227.79) -- (166.07,235.79) -- (132.36,235.79) -- cycle ;
%Pentagon Arrow [id:dp7540069236146814] 
\draw  [pattern=_yfxndt14e,pattern size=6pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (290.78,236.46) -- (257.07,236.46) -- (247.8,228.46) -- (257.07,220.45) -- (290.78,220.45) -- cycle ;
%Pentagon Arrow [id:dp18740762504693875] 
\draw  [pattern=_ad2uj7z6h,pattern size=6pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (418.86,197.78) -- (385.15,197.78) -- (375.89,189.77) -- (385.15,181.77) -- (418.86,181.77) -- cycle ;
%Pentagon Arrow [id:dp15323576786143045] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (338.01,303.16) -- (338.01,269.45) -- (346.02,260.18) -- (354.02,269.45) -- (354.02,303.16) -- cycle ;
%Pentagon Arrow [id:dp13718273298203765] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (50.67,304) -- (50.67,270.29) -- (58.67,261.02) -- (66.68,270.29) -- (66.68,304) -- cycle ;
%Pentagon Arrow [id:dp5864204849271528] 
\draw  [pattern=_3evgjc7wg,pattern size=6pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (50.67,217.49) -- (50.67,183.78) -- (58.67,174.51) -- (66.68,183.78) -- (66.68,217.49) -- cycle ;
%Curve Lines [id:da3013730012595639] 
\draw    (58.67,261.02) .. controls (59.04,216.76) and (91.75,255.34) .. (92.73,200.13) ;
\draw [shift={(92.75,197.55)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da09862002824619398] 
\draw    (24.54,201.02) .. controls (25.87,255.79) and (59.04,217.81) .. (58.67,261.02) ;
\draw [shift={(24.5,197.55)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da22060104591446938] 
\draw    (573.32,190.64) -- (573.5,235.67) ;
\draw [shift={(573.31,187.64)}, rotate = 89.78] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da290866897275299] 
\draw    (523.76,189.8) .. controls (570.29,190.98) and (516.66,290.93) .. (574.29,293.61) ;
\draw [shift={(577,293.67)}, rotate = 179.69] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Pentagon Arrow [id:dp3393473279546162] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (565.49,278.65) -- (565.49,244.94) -- (573.5,235.67) -- (581.5,244.94) -- (581.5,278.65) -- cycle ;
%Pentagon Arrow [id:dp13942391956904343] 
\draw  [pattern=_y0hgzn6lm,pattern size=6pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (480.78,181.8) -- (514.49,181.8) -- (523.76,189.8) -- (514.49,197.81) -- (480.78,197.81) -- cycle ;




\end{tikzpicture}

==> middleware_modules.tex <==
\begin{tikzpicture}[node distance=1cm and 1cm]
	\tikzstyle{boxbox} = [rectangle, minimum width=1.6cm, minimum height = 0.8cm, text centered, draw=black]
        \tikzstyle{boxboxnoborder} = [rectangle, minimum width=1.6cm, minimum height = 0.8cm, text centered]
 	\tikzstyle{boxboxinvis} = [rectangle, minimum width=1.6cm, minimum height = 0.8cm, text centered]
        \tikzstyle{boxspecial} = [rectangle, dashed, minimum width=1.6cm, minimum height = 0.8cm, text centered, draw=black]
	\tikzstyle{boxboxbig} = [rectangle, minimum width=1.6cm, minimum height = 3cm, text centered]%, draw=black]
	\tikzstyle{boxboxsmall} = [rectangle, minimum width=0.001cm, minimum height = 1cm, text centered]%, draw=black]
	
	\tikzstyle{arrow} = [thick, ->,>=stealth]
	
	
	\node (SFU) [boxbox] {SFU};
	\node (COS) [boxboxnoborder,text width=2cm, left = of SFU] {Sensory \\ information};
	\node (XBR) [boxboxinvis, above = of COS,yshift=-15] {};
	\node (IMU) [boxboxinvis, below = of COS, yshift=15] {};
	\node (AIS) [boxboxinvis, below = of IMU,yshift=11] {};
	\node (SAS) [boxbox, right  = of SFU] {SAS};
	%\node (COS) [boxbox, left of = SFU] {COS};
	%\node (SHL) [boxbox, below of = COS] {SHL};

        \node (AIS_space) [boxboxsmall, below = of AIS]{};
        \node (MWS)[boxspecial, below = of AIS_space,yshift=21.5]{MWS};
	
	\node (ANS) [boxbox, right =of SAS] {ANS};
	\node (ACS) [boxbox, below =of ANS] {ACS};
	\node (ACS_space_1) [boxboxsmall, below =of ACS] {};
	
	\node (APS) [boxbox, left =of ACS_space_1, xshift=15] {APS};
	\node (VCS) [boxbox, right =of ACS_space_1, xshift=-15] {VCS};
	\node (SHP) [boxbox, right =of ANS] {SHP};
	\node (SAS_space_1) [boxboxbig, below =of SAS] {};
	
	\node (HMI) [boxbox, below =of SAS_space_1,xshift=-0] {HMI};
	\node (HMI_SAS_arrow) [boxboxsmall, below =of SAS_space_1,xshift=-10] {};
	\node (SAS_HMI_arrow) [boxboxsmall, above = of SAS_space_1, xshift=-10] {};
	\node (RUT) [boxbox, below =of SHP] {RUT};
	%\node (RCC) [boxbox, below =of HMI] {RCC};
	
	\node (SHP_space_1) [boxboxsmall, right = of SHP,xshift=-15]{};
	\node (SHP_space_2) [boxboxsmall, below = of SHP_space_1]{};
	\node (SHP_space_3) [boxboxsmall, below = of SHP_space_2]{};
	\node (SHP_space_4) [boxboxsmall, below = of SHP_space_3,yshift=-25]{};
	\draw (SHP)--(SHP_space_1);
	\draw (SHP_space_1.west)--(SHP_space_4.west);
	\draw[arrow] (SHP_space_4)-|(HMI);
	
	%\draw[arrow](COS) -- (SFU);
	%\draw[arrow](SHL) -- (SFU);
	
	\draw[arrow](SFU) |- (HMI);
	\draw[arrow](SFU) -- (SAS);
	
	\draw[arrow](SAS) -- (ANS);
	\draw[arrow](SAS_HMI_arrow) -- (HMI_SAS_arrow);
	\draw[arrow](SAS) -- (ACS);
	
	\draw[arrow](ANS) -- (ACS);
	\draw[arrow](APS) -- (ACS);
	\draw[arrow](ACS) -- (APS);
	\draw[arrow](VCS) -- (ACS);
	\draw[arrow](ACS) -- (VCS);
	
	\draw[arrow](SHP) -- (ANS);
	\draw[arrow](ANS) -- (SHP);
	
	\draw[arrow](RUT) -- (SHP);
	\draw[arrow](RUT) |- (HMI);
	\draw[arrow](RUT) -- (ACS);
	\draw[arrow](ACS) -- (RUT);
	
	
	\draw[arrow](HMI) |- (ACS);
	
	\draw[arrow](COS) -- (SFU);
	%\draw[arrow](XBR) -- (SFU);
	%\draw[arrow](IMU) -- (SFU);
	%\draw[arrow](AIS) -- (SFU);
	
	
\end{tikzpicture}

==> shp_module_io.tex <==
\begin{tikzpicture}
    \matrix (m) [
        matrix of nodes,
        nodes in empty cells,
        nodes = {
            text height=2ex, text depth=0.5ex,
            inner sep=1mm, outer sep=0mm,
        },
        row sep = 0mm, column sep = 7mm,
        column 1/.style = {nodes={align=right, anchor=south east}},
        column 2/.style = {nodes={align=center, anchor=south, text width=13ex}}, % change width of block here
        column 3/.style = {nodes={align=left, anchor=south west}},
    ] {
    $\mathbf{x}$                           &                   &   \hl{Output!}    \\
    $\mathbf{x}_{\text{goal}}$             &                   &   \hl{Output!}  \\
    $\mathcal{X}_{\text{TV}}$              &                   &   \hl{Output!}   \\
    $\mathcal{X}_{\text{ENC}}$    &   SHP             &                   \\
    \hl{Input!}    &                   &   \hl{Output!}   \\
                    &                   &                   \\
    \hl{Input!}    &                   &                   \\
    };
    \scoped[on background layer]
        \node (enc)  [draw, rounded corners, semithick, fill=gray!10,
                      inner sep = 0mm, outer sep= 0mm,
                      fit=(m-1-2) (m-7-2)] {}; 
    \foreach    \i in {1,...,5,7}
        \draw[-{Triangle[angle=60:2pt 4]}]    (m-\i-1) -- (m-\i-2);
    \foreach    \i in {1,...,3,5}
        \draw[-{Triangle[angle=60:2pt 4]}]    (m-\i-2) -- (m-\i-3);
\end{tikzpicture}
